Outlier-Based Domain of Applicability Identification for Materials Property Prediction Models

Machine learning models have been widely applied for material property prediction. However, practical application of these models can be hindered by a lack of information about how well they will perform on previously unseen types of materials. Because machine learning model predictions depend on the quality of the available training data, different domains of the material feature space are predicted with different accuracy levels by such models. The ability to identify such domains enables the ability to find the confidence level of each prediction, to determine when and how the model should be employed depending on the prediction accuracy requirements of different tasks, and to improve the model for domains with high errors. In this work, we propose a method to find domains of applicability using a large feature space and also introduce analysis techniques to gain more insight into the detected domains and subdomains.

==> archive/deleted_text.tex <==
ABOUT FEATURE IMPORTANCE
Some of the molecular descriptors are too theoretical to easily relate them to physical or structural properties of the molecules. Therefore something we can do is to find the feature importance using more easy-to-interpret descriptors. We selected such features by inspection and used them to train a classification model using ExtraTreesClassifier as we did before. Our results are shown in Figure \ref{fig:feature-imp-difference-expl}. Once again, when taking decisions using these results, we should also compare the feature values of in-cluster and out of cluster molecules. These results are shown in Figure \ref{fig:feature-imp-difference-expl}.

To identify the prominent features of others, we follow a method 
described at Reference \cite{Alghofaili_2021}. Using a random forest classification model, which has the ability to identify feature importances, we train models to separately identify members of a selected cluster from the members of all the other clusters combined. The resulting feature importance values shown by the blue bars in Figure \ref{fig:feature-imp-difference-expl} tell us which features played a major role in helping the model distinguish the selected cluster from the other clusters. 

However, there is no guarantee that the descriptors shown in Figure \ref{fig:feature-imp-difference-expl} are the ones we can use to distinguish them from the other molecules. \textcolor{nc}{This is because, the classifier might find the features that a more prominent in the class we are not interested in.} We MinMax scaled the descriptors and found the averages of descriptors of molecules belonging to a cluster and the rest of the molecules. As shown in Figure \ref{fig:feature-imp-difference-expl}, we see that in most of the cases the important descriptors determined by ExtraTreesRegressor distinguish the molecules in a given group. However there are exceptions. For cluster 6, the most important descriptors seem to be the dominant descriptors of molecules which do not belong to the cluster. Therefore, one should use both these results when trying to understand the unique characteristics of molecules in these groups. 

These methods allow us to find the probability that a molecule is an outlier or an inlier. Using these probabilities we determined whether each molecules can be classified as an outlier or inlier.

As the domain index increases, the number of molecules inside the domain increases and the number of molecules outside the domain decreases.



In Table \ref{table:data-str-ols}, we summarize the properties of different types of outliers and inliers. Interestingly a significant percentage of data outliers contains chiral centers and have an isomer counterpart. \textcolor{red}{These numbers don't look that significant compared to the IL. Are these the most significant factors you found?}. We think that this fact reveals the reasons for having data outliers. That is, the ML modeling we use lacks the ability to understand structure-property relationships of molecules containing chiral centers. Also, our models find it difficult to make accurate predictions when there are structurally similar molecules.


\begin{table}[tbh]
\centering
\small
\caption{Number of molecules in outliers, inliers, structural outliers and data outliers having different properties. The numbers are given as a percentage of the total number of molecules in each group. nAtom stands for number of atoms in the molecule. BertzCT is a molecular descriptor that attempts to measure the complexity of the molecule.}

\begin{tabular}{lrrrr}
\toprule
                   Property &  STR.OL  &  DATA.OL  &    ALL.OL  &  IL \\
\midrule
                     Count &          1013 &    3033 & 4046 &  16183 \\

                nAtom $>$ 100 &            17.18 \% &       1.12 \% &    5.14 \% &      0.61 \% \\
             BertzCT $>$ 1500 &            21.52 \% &       1.09 \% &    6.20 \% &      1.22 \% \\
            Chiral centers &            19.94 \% &      10.19 \% &   12.63\% &      9.87 \% \\
Have an isomer counterpart  &            16.78 \% &      12.96 \% &   13.91 \% &     11.88 \% \\
\bottomrule
\end{tabular}
\label{table:data-str-ols}
\end{table}







Next, we observe how the performance of the solubility prediction models changes after removing outliers selected using different methods. In Table \ref{table:cv_nol_diff_methods}, we list the accuracies obtained by existing anomaly detection methods and the solubility-aware outlier detection method. 
The number of outliers removed is approximately 15\% of the total number of molecules. 


In this section, we propose two supervised outlier detection methods. One is based on training a classifier and the other on the outlierness associated with molecules.

To demonstrate these processes, we first split our dataset into train and test folds. Prediction errors for each molecule in the train set are calculated as explained in the section A. Next we used the same method which we used in section A to separate outliers and inliers. Outlier percentage we consider is 20\% of the train-validation set.





\begin{table}[tbh]
\centering
\small
\caption{References corresponding to data outliers with largerst outlierness}

\begin{tabular}{lr}
\toprule
                                            ExpRef &  olness \\
\midrule
                         LETINSKI.DJ ET AL. (2002) &    0.42 \\
Bulletin\_de\_la\_Societe\_Chimique\_de\_France;\_(195... &    0.39 \\
Staverman. A.J.. Ph. D. thesis. University of L... &    0.38 \\
                             YAWS.CL ET AL. (2001) &    0.37 \\
                            COATES.M ET AL. (1985) &    0.35 \\
Schreiber;\_Chemische\_Berichte;\_vol.\_57;\_(1924);... &    0.33 \\
                                MERCK INDEX (2013) &    0.27 \\
                                  SEIDELL.A (1941) &    0.27 \\
                                  TOMLIN.C (1997) &    0.26 \\
                                 PARRISH.CF (1983) &    0.26 \\
\bottomrule
\end{tabular}

\label{table:ref_olness}
% EA-error-analysis-CHEM
\end{table}



Before finding the differences, we have scaled each descriptor such that the largest value is equal to one and the smallest equal to zero (MinMax scaling). 

It is unknown how intramolecular H-bonds may impact solubility, but the formation of them can remove potential polar groups from interacting with water or restrict the movement/free rotation of molecule bonds. It is anticipated that these intramolecular interactions, within a single molecule, should be captured by the machine learning model. 

\textbf{Long Alkyl Chains.} Long alkyl chains will undergo hydrophobic collapse when dissolved in water and as a result of the high number of rotatable bonds there will be 2(to the powerof)n number of possible conformations that could be present. However, the machine learning model does not take into account these different conformations when determining the solubility and is therefore looking at an inaccurate description of the molecule that is in solution. A common subset of these alkyl chains are perfluorinated alkanes, where the hydrogens have been replaced by fluorines. These can also undergo hydrophobic collapse. In addition they are known(ref) to be less soluble than their hydrocarbon counterparts in aqueous solution.


% \begin{table}[tbh]
% \centering
% \small
% \caption{CV scores obtained for PNNL dataset by recent models.}
% \begin{tabular}{lrr}
% \toprule
%   Method &  RMSE &   R2 \\
% \midrule
%      ETR &  1.06 & 0.78 \\
%      CBM &  1.06 & 0.78 \\
%      RF &  1.07 & 0.78 \\
%     XGB &  1.09 & 0.77 \\
%     LGB &  1.10 & 0.77 \\
%     AttentiveFP &  1.11 & 0.76 \\
%      SVM &  1.13 & 0.75 \\
% GNN-fgrp &  1.15 & 0.75 \\
%  GNN-reg &  1.15 & 0.75 \\
%      MDM &  1.15 & 0.74 \\
%      GBR &  1.20 & 0.72 \\
% \bottomrule
% \end{tabular}
% \label{table:curr-preds}
% % EA-error-analysis-CHEM
% \end{table}













% \begin{table}[tbh]
% \centering
% \footnotesize
% \caption{CV scores obtained for inliers  predicted by different anomaly detection methods. ExtratreesRegressor has been used as the ML model.}


% \begin{tabular}{lllr}
% \toprule
%                                   Methods &         RMSE &           R2 &   olp \\
% \midrule
%                               Solubility-aware & 0.54 pm 0.01 &  0.92 pm 0.0 & 20.00 \\
%                           Isolation Forest & 0.83 pm 0.03 & 0.82 pm 0.01 & 20.00 \\
%   Histogram-base Outlier Detection (HBOS) & 0.85 pm 0.02 & 0.81 pm 0.01 & 20.00 \\
%                  K Nearest Neighbors (KNN) & 0.85 pm 0.01 &  0.83 pm 0.0 & 18.14 \\
%       Angle-based Outlier Detector (ABOD) & 0.86 pm 0.02 & 0.83 pm 0.01 & 21.27 \\
%                      One-class SVM (OCSVM) & 0.86 pm 0.03 & 0.82 pm 0.01 & 20.00 \\
%         Principal Component Analysis (PCA) & 0.86 pm 0.02 & 0.81 pm 0.01 & 20.00 \\
%                           Feature Bagging & 0.87 pm 0.01 &  0.83 pm 0.0 & 18.69 \\
%                 Local Outlier Factor (LOF) & 0.87 pm 0.04 & 0.83 pm 0.01 & 18.74 \\
% Cluster-based Local Outlier Factor (CBLOF) & 0.88 pm 0.02 & 0.81 pm 0.01 & 20.00 \\
%       Minimum Covariance Determinant (MCD) & 0.89 pm 0.02 & 0.82 pm 0.01 & 20.00 \\
% \bottomrule
% \end{tabular}
% \label{table:cv_nol_diff_methods}
% \end{table}


% \begin{table}[tbh]
% \centering
% \small
% \caption{CV scores obtained using different ML models for inliers determined by solubility-aware method.}
% \begin{tabular}{l|rr}
% \toprule
%  \textbf{\small{Model}} &  \textbf{\small{RMSE}} &  \textbf{\small{$R^2$}} \\
% \midrule
%  Random Forest &  A &   A \\
%  MLP &  A &   A \\
%  GNN &  A &   A \\
%  LGB &  0.61 &   0.91 \\
 
% \bottomrule
% \end{tabular}
% \label{table:cv-nol-models}
% % EA-error-analysis-CHEM
% \end{table}


% \subsection{Domains of Applicability}

% \subsubsection{Training a Classifier to Predict Outliers}


% \begin{table}
% \centering
% \small
% \caption{Solubility prediction accuracies when outliers are removed from train or test and train+test folds.}

% \begin{tabular}{lrr}
% \toprule
% Outliers removed from &  RMSE &   R2 \\
% \midrule
%           Train+Test &  0.89 & 0.81 \\
%             Test only &  0.85 & 0.82 \\
%           Train only &  1.19 & 0.73 \\
% \bottomrule
% \end{tabular}

% \label{table:remove-ols-pnnl}
% \end{table}



% \begin{table*}
% \centering
% \tiny
% \caption{RMSE and R2 for inlier test molecules selected by different methods.
% K Nearest Neighbors (KNN), Principal Component Analysis (PCA), One-class SVM (OCSVM),Isolation Forest (IF), Angle-based Outlier Detector (ABOD), Cluster-based Local Outlier Factor (CBLOF), Feature Bagging (FB), Histogram-base Outlier Detection (HBOS), Minimum Covariance Determinant (MCD), Local Outlier Factor (LOF)
% }

% \begin{tabular}{lrr|rr}
% \toprule
% & \multicolumn{2}{c|}{Remove from test only} &\multicolumn{2}{c}{Remove from test+train} \\
%                                       meth &  rmse &  r2 &  rmse &   r2 \\
% \midrule
%                                       pnnl &       0.85 &     0.82 &  0.89 & 0.81 \\
%                  K Nearest Neighbors (KNN) &       0.86 &     0.84 &  0.88 & 0.83 \\
%                      One-class SVM (OCSVM) &       0.86 &     0.81 &  0.88 & 0.80 \\
%                           Isolation Forest &       0.86 &     0.80 &  0.88 & 0.80 \\
%         Principal Component Analysis (PCA) &       0.88 &     0.80 &  0.88 & 0.80 \\
%                 Local Outlier Factor (LOF) &       0.89 &     0.82 &  0.91 & 0.81 \\
%   Histogram-base Outlier Detection (HBOS) &       0.89 &     0.80 &  0.91 & 0.79 \\
%       Angle-based Outlier Detector (ABOD) &       0.89 &     0.82 &  0.90 & 0.82 \\
%                           Feature Bagging &       0.90 &     0.82 &  0.90 & 0.82 \\
%       Minimum Covariance Determinant (MCD) &       0.90 &     0.82 &  0.89 & 0.82 \\
% Cluster-based Local Outlier Factor (CBLOF) &       0.90 &     0.79 &  0.91 & 0.79 \\
%                               Average KNN &       0.95 &     0.81 &  0.98 & 0.80 \\
% \bottomrule
% \end{tabular}

% \label{table:remove-ols-from-test}
% % EA-error-analysis-CHEM
% \end{table*}



% \begin{table}
% \centering
% \small
% \caption{RMSE and R2 when both pnnl and pyod outliers are removed from the test set.
% }
% \begin{tabular}{lrrr}
% \toprule
%     Method &  RMSE &   R2 &  \#ol\_test \\
% \midrule
%                  K Nearest Neighbors (KNN) &  0.77 & 0.84 &       396 \\
%       Angle-based Outlier Detector (ABOD) &  0.78 & 0.85 &       468 \\
%                 Local Outlier Factor (LOF) &  0.78 & 0.84 &       420 \\
%                           Feature Bagging &  0.78 & 0.84 &       424 \\
%       Minimum Covariance Determinant (MCD) &  0.80 & 0.84 &       421 \\
%                               Average KNN &  0.81 & 0.83 &       296 \\
% Cluster-based Local Outlier Factor (CBLOF) &  0.81 & 0.81 &       418 \\
%                      One-class SVM (OCSVM) &  0.82 & 0.81 &       408 \\
%         Principal Component Analysis (PCA) &  0.82 & 0.81 &       403 \\
%   Histogram-base Outlier Detection (HBOS) &  0.82 & 0.81 &       382 \\
%                           Isolation Forest &  0.83 & 0.81 &       376 \\
% \bottomrule
% \end{tabular}

% \label{table:rem-ols-pnnl-pyod}
% \end{table}


% \subsubsection{Gaining Insight on Detected Outliers and Inliers}
% In this section, we are going to analyse the proprties of outliers and inliners in detail.


% \begin{table}[tbh]
% \centering
% \small
% \caption{Number of molecules in outliers and inliers,  having different properties. The numbers are given as a percentage of the total number of molecules in each group.}
% \begin{tabular}{lrr}
% \toprule
%                   Property &  Outliers &  Inliers  \\
% \midrule
%              Chiral centers &     14.16 &     9.79 \\
%               nAtom $>$ 100 &      5.33 &     0.54 \\
%           BertzCT $>$ 1500 &      6.53 &     1.13 \\
% Have an isomer counterpart  &     16.26 &    11.04 \\
% \bottomrule
% \end{tabular}
% \label{table:ol_nol_diff1}
% % EA-error-analysis-CHEM
% \end{table}


% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=1\textwidth]{images/unsup/clusters/image_groups.png}
    
%     \caption{Clusters of outlier molecules.}
%     \label{fig:mol-clusters}
% \end{figure*}

% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[width=1\textwidth]{images/unsup/clusters/cluster_fimp.png}
    
%     \caption{Clusters feature importance}
%     \label{fig:mol-clusters-2}
% \end{figure*}






% \begin{table}[tbh]
% \centering
% \small
% \caption{Number of molecules in outliers, inliers, structural outliers and data outliers having different properties. The numbers are given as a percentage of the total number of molecules in each group.}

% \begin{tabular}{lrrr}
% \toprule
%                   Property &  Structural OL &  Data OL  &  Inlier  \\
% \midrule
%              Chiral centers &          15.58 &      9.78 &     9.79 \\
%               nAtom $>$ 100 &           7.06 &      0.00 &     0.54 \\
%           BertzCT $>$ 1500 &           8.65 &      0.00 &     1.13 \\
% Have an isomer counterpart  &          14.67 &     21.16 &    11.04 \\
% \bottomrule
% \end{tabular}

% \label{table:CV_LIT}
% % EA-error-analysis-CHEM
% \end{table}


% \begin{figure*}[!t]
%      \centering
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/unsup/data_ol/n_similar_pairs.png}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/unsup/data_ol/diff_vs_simth.png}
%      \end{subfigure}
%     \caption{ (a) Distribution of average solubility differences corresponding to molecule pairs that are $>$0.99 similar. (b) Mean solubility difference between nearest neighbors versus the similarity threshold.}
%         \label{fig:data-ol}
% \end{figure*}





% \begin{table}[tbh]
% \centering
% \begin{tabular}{lrrrrrr}
% \toprule
% prop &  lower\_pnnl &  upper\_pnnl &  lower\_delaney &  upper\_delaney &  lower\_cui &  upper\_cui \\
% \midrule
%   NssssSn &        0.00 &        0.00 &           0.00 &           0.00 &       0.00 &       0.00 \\
%       Mpe &        0.87 &        1.34 &           0.89 &           1.34 &       0.78 &       1.37 \\
%       IC2 &        0.72 &        5.45 &           0.72 &           5.27 &      -0.00 &       6.14 \\
% n10AHRing &        0.00 &        0.00 &           0.00 &           0.00 &       0.00 &       0.00 \\
%       IC3 &        0.72 &        6.05 &           0.72 &           5.71 &      -0.00 &       6.86 \\
%      bpol &        2.01 &       55.53 &           2.01 &          77.23 &       0.00 &     149.23 \\
%       IC5 &        0.72 &        6.22 &           0.72 &           6.00 &      -0.00 &       7.22 \\
%      CIC0 &        0.40 &        5.52 &           0.40 &           5.05 &       0.00 &       5.73 \\
%       n6 &        0.00 &        2.00 &           0.00 &           0.00 &       0.00 &       0.00 \\
%  SMR\_VSA7 &        0.00 &      149.19 &           0.00 &          95.05 &       0.00 &     216.38 \\
%       n5 &        0.00 &        4.00 &           0.00 &           0.00 &       0.00 &      19.00 \\
%   BertzCT &        0.00 &     1552.14 &           0.00 &        1140.95 &       0.00 &    4709.88 \\
%  BalabanJ &        0.00 &        4.65 &           0.00 &           4.65 &      -0.00 &       5.50 \\
%     piPC2 &        0.00 &        4.73 &           0.00 &           4.73 &       0.00 &       5.09 \\
%      Mare &        0.90 &        1.35 &           0.90 &           1.35 &       0.90 &       1.43 \\
% \bottomrule
% \end{tabular}

% \label{table:doa_ext}
% % EA-error-analysis-CHEM
% \end{table}


% The molecules having anomaly scores less than or equal to this anomaly score were chosen to evaluate the anomaly detection method. That is, we randomly split these molecules as train and test molecules (80/20 ratio). We fit an ExtraTreesRegressor model using the train set and found the R2 score for the test set. These R2 scores were recorded for each anomaly detection method. The 20 methods having the largest R2 scores were selected as the final anomaly detection methods. 

% \subsection{\textbf{More insight on in-domain and out-of-domain molecules}}\label{sec:doa-select}
% Our domains are well defined using the molecular properties.
% We can gain more insight about these molecules using cluster analysis - such as, are there groups of molecules with similar properties and what are pronounced molecular descriptors of these groups.
% \subsubsection{Properties of structural outliers}


\textcolor{nc}{To demonstrate how we can use the knowledge on in-doman and out-of-domain molecules gain more insight about them, we discuss two examples. In the first case, after visual inspection of some outliers, we hypothesized that the presence of intra-molecular Hydrogen bonds could be a cause for the existence of some data outliers. Kuhn and coworkers have provided a criterion to intra-molecular hydrogen bonds in organic molecules \cite{Kuhn2010}. We used the same criterion to detect the molecules with intra-molecular hydrogen bonds in our dataset.}

\textcolor{nc}{Another hypothesis is that as the length of the carbon chain increases, there is a possibility for them to fold. This phenomenon is observed in polymers and protein structures. Molecules with folded carbon chains can result in low solubilities. Such folding can occur in molecules when there are rotatable bonds. From Figure \ref{fig:feature-imp-difference-expl}, we can see that molecules in Group 5 consists of more rotational bonds compared to other structures. Out of the molecules we considered to obtain clusters in Figure \ref{fig:ood-groups}, 4\% of Group 10 molecules are inliers, 13\% are outliers, 4\% are structural outliers,
7\% are data outliers and 2\% are structural anomalies. Even though not conclusive, we think that this kind of analysis using the molecules in domains and subdomains can be helpful to figure out the causes of current limitations in our models.
}

\begin{figure*}[!t]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intraH/example_ab.png}
         \caption{}
         % \label{fig:diff-vs-sim}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/intraH/example_c.png}
         \caption{}
     \end{subfigure}
        \caption{Examples of molecules in which intra-molecular Hydrogen bonds can exist.}
        \label{fig:}
\end{figure*}




\begin{table}[!htb]
\caption{Number of molecules with possible intra-molecular Hydrogen bonding sites
as percentage of all the train data.
}
\centering

\begin{tabular}{lc}
\toprule
    Data type &  \% of IntraH \\
\midrule
      STR.OL &         0.13 \\
     DATA.OL &         0.28 \\
   STR.ANMLY &         0.05 \\
ALL.OL (NEW) &         0.46 \\
ALL.IL (NEW) &         0.57 \\
ALL.OL (OLD) &         0.41 \\
ALL.IL (OLD) &         0.63 \\
\bottomrule
\end{tabular}


\label{table:}
\end{table}

However, to confirm the validity of this test, we should have solubility values for the chosen `test' set. Hence, for this purpose, we used the PNNL test set which was not used in the DoA determining process.

